Using Contextually Aligned Online Reviews to Measure LLMs' Performance Disparities Across Language Varieties

A language can have different varieties. These varieties can affect the performance of natural language processing (NLP) models, including large language models (LLMs), which are often trained on data from widely spoken varieties. This paper introduces a novel and cost-effective approach to benchmark model performance across language varieties. We argue that international online review platforms, such as Booking.com, can serve as effective data sources for constructing datasets that capture comments in different language varieties from similar real-world scenarios, like reviews for the same hotel with the same rating using the same language (e.g., Mandarin Chinese) but different language varieties (e.g., Taiwan Mandarin, Mainland Mandarin). To prove this concept, we constructed a contextually aligned dataset comprising reviews in Taiwan Mandarin and Mainland Mandarin and tested six LLMs in a sentiment analysis task. Our results show that LLMs consistently underperform in Taiwan Mandarin.

==> sections/deleted/2-1-eval-peroformance-gap.tex <==
%\kenneth{Did people compare NLP models' performances across language variations? How? What did they find? Why can (or can not) their methods be used in our case?}

%\zixin{Here are several existing benchmarks specifically for language variation/diversity}
%\kenneth{Cool. Say a few words about what these benchmarks did? How do they compare model performance across variations?}
%\zixin{What about tasks directly focus on detecting language variation? i.e. dialect detection and identification? I just separated those papers from other benches so we can discuss them later.}\kenneth{In our setting, we kinda KNOW the variation of each data item, as Booking.com has users' self-reported nationality/region. So, variation detection is a separate problem-- it might be useful when, say, your data don't tell you the variations, so you need to detect them yourself.}

%\zixin{I found this 2020 ACL paper discussing several "missing parts" NLP studies on "biases", including related work outside of NLP tasks and communities. It might be worth taking a look}
%\cite{blodgett2020biasreview}


%General NLP benchmarks for language variations/diversity: DIALECTBENCH~\cite{dialectbench}, VALUE (Specific for African American English~\cite{valuebench}), Macuco corpus \cite{macucocorpus}


%\paragraph{CAMP 1: Compared or aligned using NLP tasks.}
%DIALECTBENCH~\cite{dialectbench}:
%Collect a set of languages and put them in the same leaderboard





%\kenneth{Bad: It's not really a fair or even comparable comparison.}

%\paragraph{CAMP 2: Compared or aligned using data (direct conversion at the instance level).}

%VALUE~\cite{valuebench}:
%Use rule-based approaches to convert MAE to AAE and eval on AAE. The conversation was validated by humans!

%Multi-VALUE~\cite{multivaluebench}:
%Extended version of VALUE to 50 dialects with 189 linguistic features, and synthetic mapping to SAE. Native speakers verified several dialects.

%\kenneth{Bad: Conversion is hard or expensive}








%\cite{hovy-johannsen-2016-exploring}

%\kenneth{This is one paper I found, which has a whole ``Language Variation'' subsection. Maybe take a look:}
%\cite{lwowski2022measuring}

%\kenneth{Did people compare NLP models' performances across different languages? How? What did they find? Why can (or can not) their methods be used in our case?}


%\kenneth{Now when I think about it, we can also learn some methods from people who work on biases in AI models on how they compare AI models' performances gap across different user populations}

%\paragraph{scenario-based studies for biases in AI models regarding language variations}

%Case study for AAE tweets~\cite{AAE2017racial}: This case study investigated models' performance gap on language identification tasks regarding AAE and SAE tweets. Results showed gaps in identifying AAE short tweets as English, indicating potential biases against minority language users in large-scale models training on major language variation.

%\textbf{Method:} Language identification tasks (whether it is an English tweet) on AAE and SAE tweets

%\citeauthor{groenwold2020AAENLP}: Using parallel AAVE/SAE tweet prompts and GPT-2, researchers found a consistent disparity in AAVE-like generation, including the sentiment analysis scores, benchmark scores on BLUE and ROUGE, and human-based evaluation on generated text quality. 

%\textbf{Method:} stat. analyses on benchmark scores (sentiment, BLUE, ROUGE) and human evaluations regarding NLG output.

%\citeauthor{liang2023gptesl}: Compared to essays from 8th-grade native speakers, non-native English essays have a higher chance of being classified as "AI-generated" by GPT-based detectors (ChatGPT in this case). Such issues can be reduced by enhancing word choices in the essays, indicating that such a biased pattern is related to linguistic diversity in language production.

%\textbf{Method:} Ratio of "AI-generated" labels regarding non-native essays and essays from 8th-grade students.

%\citeauthor{kwako2023bertbias}: This study investigated BERT's performance of rating transcripts of non-native speakers' speeches, and whether BERT can perform similar patterns as humans when conducting the same tasks. Results showed that BERT may exacerbate the difference against different non-native speakers groups, indicating potentially stronger implicit biases in BERT. Such rating differences are larger if the speaker is older or speaks longer. 

%\textbf{Method:} auto-grading system based on off-the-shelf BERT(so zero-shot I guess?), and the differences between humans' and BERT's scores are represented as differential item functioning (DIF)


%Macuco corpus~\cite{macucocorpus}:
%A parallel data for multiple English variations in Europe. Includes only variation identification tasks.


==> sections/deleted/2-2-Chinese-NLP.tex <==
%\kenneth{Maybe need to mention the efforts of creating localized LLMs for China and Taiwan, respectively.}

%\kenneth{Discuss how some shared tasks, e.g., NTCIR-6, sometimes have BOTH China and Taiwan Mandarin subset. Like this: https://research.nii.ac.jp/ntcir/permission/ntcir-6/perm-en-OPINION.html}

%\kenneth{Maybe discuss the shared tasks in SIGHAN: https://dimabsa2024.github.io/}

%\paragraph{Related work on Chinese NLP: Fine-tuning dataset}

%COIG-CQIA ~\cite{bai2024coig}:
%A large fine-tuning instruction dataset for LLMs, contains various types of data including Wikis, examinations, professional documents, and online Q\&A community threads. However, most of the data comes from mainland China, which might introduce biases against other great Chinese region users.


%\paragraph{Direct NLP tasks/datasets for identifying and detecting language variation}

%2019 VarDial Evaluation Campaign~\cite{vardial2019report}:
%Dataset for various types of language variation NLP tasks, including dialect identification and cross-lingual morphological analysis tasks. It also includes a dataset for discriminating Taiwan and Mainland variations of Chinese under the same scripts/orthography system. 
%\zixin{Can we borrow similar ideas of using the same writing script system for both language variations?}\kenneth{When we justify our method of comparing TW Mandarin and China Mandarin, yes? I'd move this to Chinese NLP subsection though.}




==> table/main-result-table.tex <==

\sisetup{print-zero-integer=false}

\begin{table*}[t]
\centering
\small
\addtolength{\tabcolsep}{-1.2mm}
\begin{tabular}{
    @{}ll
    S[table-format = .3, table-space-text-post = $^{***}$] S[table-format = 0.3]
    S[table-format = .3, table-space-text-post = $^{***}$] S[table-format = 0.3]
    S[table-format = .3, table-space-text-post = $^{***}$] S[table-format = 0.3]
    S[table-format = 1.3, table-space-text-post = $^{***}$] S[table-format = 1.3]
    S[table-format = 1.3, table-space-text-post = $^{***}$] S[table-format = 1.3]
    S[table-format = 1.3, table-space-text-post = $^{***}$] S[table-format = 1.3]@{}
    % ccccccccccc@{}
}
% S[table-format = 2.3, table-space-text-post = $^{***}$]
\toprule
\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Text\\ Length\\ (\#word)\end{tabular}}} & \multirow{3}{*}{\textbf{Model}} & \multicolumn{6}{c}{\textbf{ACC} $\uparrow$} & \multicolumn{6}{c}{\textbf{MSE} $\downarrow$} \\ \cmidrule(lr){3-8} \cmidrule(lr){9-14}
 &  & \multicolumn{2}{c}{\textbf{structured}} & \multicolumn{2}{c}{\textbf{plain}} & \multicolumn{2}{c}{\textbf{shuffled}} & \multicolumn{2}{c}{\textbf{structured}} & \multicolumn{2}{c}{\textbf{plain}} & \multicolumn{2}{c}{\textbf{shuffled}} \\ \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12} \cmidrule(lr){13-14}
 &  & \textbf{tw} & \textbf{cn} & \textbf{tw} & \textbf{cn} & \textbf{tw} & \textbf{cn} & \textbf{tw} & \textbf{cn} & \textbf{tw} & \textbf{cn} & \textbf{tw} & \textbf{cn} \\ \midrule

 
\multirow{6}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Short\\ (1-49)\end{tabular}}} 
 & \textbf{GPT-4o} & \cellcolor{lightred}.265 & .274 & \cellcolor{lightred}.192$^{***}$ & .208 & \cellcolor{lightred}.186$^{***}$ & .202 & 3.563$^{*}$ & \cellcolor{lightred}3.769 & \cellcolor{lightred}4.092$^{***}$ & 3.385 & \cellcolor{lightred}4.347$^{***}$ & 3.561 \\
 % & \textbf{GPT-4o +T} & .291 & \cellcolor{lightred}.286 & \cellcolor{lightred}.213 & .217 & \cellcolor{lightred}.206 & .214 & \cellcolor{lightred}2.280 & 2.252 & \cellcolor{lightred}3.035$^{*}$ & 2.618 & \cellcolor{lightred}3.130$^{*}$ & 2.749 \\
 & \textbf{Llama3 8b} & .234$^{***}$ &\cellcolor{lightred}.216 & \cellcolor{lightred}.176 & .184 & \cellcolor{lightred}.162 & .169 & 3.402$^{***}$ & \cellcolor{lightred}3.931 & \cellcolor{lightred}3.059$^{***}$ & 2.851 & \cellcolor{lightred}3.220$^{**}$ & 3.071 \\
 & \textbf{Llama3 70b} & \cellcolor{lightred}.392 & .399 & \cellcolor{lightred}.297$^{**}$ & .310 & \cellcolor{lightred}.288$^{***}$ & .310 & \cellcolor{lightred}1.785$^{**}$ & 1.661 & \cellcolor{lightred}3.465$^{***}$ & 3.005 & \cellcolor{lightred}3.427$^{***}$ & 2.941 \\
 & \textbf{Llama3 405b} & \cellcolor{lightred}.386$^{***}$ & .412 & \cellcolor{lightred}.283$^{***}$ & .315 & \cellcolor{lightred}.290$^{***}$ & .322 & \cellcolor{lightred}2.605$^{**}$ & 2.430 & \cellcolor{lightred}4.365$^{***}$ & 3.598 & \cellcolor{lightred}4.355$^{***}$ & 3.612 \\
 & \textbf{Gemma2 9b} & .150$^{**}$ & \cellcolor{lightred}.138 & \cellcolor{lightred}.182$^{*}$ & .193 & \cellcolor{lightred}.171$^{**}$ & .184 & 2.987$^{***}$ & \cellcolor{lightred}3.168 & \cellcolor{lightred}4.089$^{***}$ & 3.367 & \cellcolor{lightred}4.462$^{***}$ & 3.646 \\
 & \textbf{Gemma2 27b} & .109 & .109 & \cellcolor{lightred}.122 & .124 & \cellcolor{lightred}.122 & .127 & \cellcolor{lightred}5.399$^{***}$ & 5.120 & \cellcolor{lightred}6.150$^{***}$ & 5.292 & \cellcolor{lightred}5.880$^{***}$ & 5.183 \\ \midrule

 
\multirow{6}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Long\\ (50+)\end{tabular}}} 
 & \textbf{GPT-4o} & \cellcolor{lightred}.356$^{***}$ & .384 & \cellcolor{lightred}.281$^{***}$ & .332 & \cellcolor{lightred}.267$^{***}$ & .314 & \cellcolor{lightred}1.846$^{***}$ & 1.577 & \cellcolor{lightred}1.834$^{***}$ & 1.570 & \cellcolor{lightred}2.070$^{***}$ & 1.743 \\
 % & \textbf{GPT-4o +T} & \cellcolor{lightred}.321$^{**}$ & .336 & \cellcolor{lightred}.262$^{*}$ & .283 & \cellcolor{lightred}.248$^{*}$ & .273 & \cellcolor{lightred}1.595$^{*}$ & 1.453 & \cellcolor{lightred}1.741$^{*}$ & 1.621 & \cellcolor{lightred}1.881$^{*}$ & 1.743 \\
 & \textbf{Llama3 8b} & \cellcolor{lightred}.224 & .228 & \cellcolor{lightred}.189$^{***}$ & .214 & \cellcolor{lightred}.179$^{***}$ & .200 & 1.895 & \cellcolor{lightred}1.901 & \cellcolor{lightred}2.024$^{***}$ & 1.835 & \cellcolor{lightred}2.111$^{***}$ & 1.933 \\
 & \textbf{Llama3 70b} & \cellcolor{lightred}.409$^{***}$ & .435 & \cellcolor{lightred}.373$^{*}$ & .391 & \cellcolor{lightred}.360$^{***}$ & .388 & \cellcolor{lightred}1.424$^{**}$ & 1.284 & \cellcolor{lightred}1.667$^{*}$ & 1.557 & \cellcolor{lightred}1.771$^{**}$ & 1.608 \\
 & \textbf{Llama3 405b} & \cellcolor{lightred}.380$^{***}$ & .410 & \cellcolor{lightred}.371$^{**}$ & .396 & \cellcolor{lightred}.357$^{***}$ & .384 & \cellcolor{lightred}1.866$^{***}$ & 1.627 & \cellcolor{lightred}1.906$^{**}$ & 1.719 & \cellcolor{lightred}2.052$^{***}$ & 1.844 \\
 & \textbf{Gemma2 9b} & \cellcolor{lightred}.142 & .151 & \cellcolor{lightred}.192$^{**}$ & .209 & \cellcolor{lightred}.174$^{*}$ & .188 & \cellcolor{lightred}2.515$^{***}$ & 2.350 & \cellcolor{lightred}2.144$^{***}$ & 1.979 & \cellcolor{lightred}2.399$^{***}$ & 2.193 \\
 & \textbf{Gemma2 27b} & .096 & \cellcolor{lightred}.092 & .077 & \cellcolor{lightred}.075 & \cellcolor{lightred}.079 & .083 & \cellcolor{lightred}5.135$^{**}$ & 4.919 & \cellcolor{lightred}5.913$^{**}$ & 5.578 & \cellcolor{lightred}5.606$^{***}$ & 5.160 \\ \midrule

 
\multirow{6}{*}{\textbf{Overall}} 
 & \textbf{GPT-4o} & \cellcolor{lightred}.296$^{***}$ & .312 & \cellcolor{lightred}.222$^{***}$ & .250 & \cellcolor{lightred}.213$^{***}$ & .240 & 2.978 & \cellcolor{lightred}3.022 & \cellcolor{lightred}3.323$^{***}$ & 2.767 & \cellcolor{lightred}3.571$^{***}$ & 2.942 \\
 % & \textbf{GPT-4o +T} & \cellcolor{lightred}.302 & .303 & \cellcolor{lightred}.231$^{**}$ & .240 & \cellcolor{lightred}.221$^{*}$ & .235 & \cellcolor{lightred}2.036$^{**}$ & 1.969 & \cellcolor{lightred}2.574$^{*}$ & 2.264 & \cellcolor{lightred}2.685$^{*}$ & 2.390 \\
 & \textbf{Llama3 8b} & .230$^{*}$ & \cellcolor{lightred}.221 & \cellcolor{lightred}.181$^{***}$ & .195 & \cellcolor{lightred}.168$^{***}$ & .181 & 2.838$^{***}$ & \cellcolor{lightred}3.170 & \cellcolor{lightred}2.672$^{***}$ & 2.470 & \cellcolor{lightred}2.806$^{***}$ & 2.644 \\
 & \textbf{Llama3 70b} & \cellcolor{lightred}.398$^{**}$ & .412 & \cellcolor{lightred}.324$^{***}$ & .339 & \cellcolor{lightred}.313$^{***}$ & .337 & \cellcolor{lightred}1.658$^{***}$ & 1.529 & \cellcolor{lightred}2.835$^{***}$ & 2.496 & \cellcolor{lightred}2.847$^{***}$ & 2.473 \\
 & \textbf{Llama3 405b} & \cellcolor{lightred}.384$^{***}$ & .411 & \cellcolor{lightred}.314$^{***}$ & .344 & \cellcolor{lightred}.313$^{***}$ & .344 & \cellcolor{lightred}2.347$^{***}$ & 2.148 & \cellcolor{lightred}3.505$^{***}$ & 2.939 & \cellcolor{lightred}3.550$^{***}$ & 2.992 \\
 & \textbf{Gemma2 9b} & .147 & \cellcolor{lightred}.143 & \cellcolor{lightred}.185$^{***}$ & .199 & \cellcolor{lightred}.172$^{***}$ & .186 & 2.823 & \cellcolor{lightred}2.882 & \cellcolor{lightred}3.410$^{***}$ & 2.881 & \cellcolor{lightred}3.742$^{***}$ & 3.137 \\
 & \textbf{Gemma2 27b} & .105 & \cellcolor{lightred}.103 & \cellcolor{lightred}.106 & .107 & \cellcolor{lightred}.107 & .111 & \cellcolor{lightred}5.307$^{***}$ & 5.049 & \cellcolor{lightred}6.067$^{***}$ & 5.392 & \cellcolor{lightred}5.785$^{***}$ & 5.175 \\ \bottomrule
 %\multicolumn{14}{l}{\textit{Statistical group differences are indicated as ${^{*}}$  (p<.05), ${^{**}}$ (p<.01), and ${^{***}}$ (p<.001) regarding the model performance.}}
\end{tabular}

\addtolength{\tabcolsep}{+1.2mm}
\vspace{-.5pc}
\caption{Results by length for GPT-4o, Llama3 (8b, 70b, 405b), and Gemma2 (9b, 27b) models. Red cells indicate a worse performance than the other group. (Statistical group differences are indicated as ${^{*}}$  (p<.05), ${^{**}}$ (p<.01), and ${^{***}}$ (p<.001) regarding the model performance.)\kenneth{TODO: (1) This table needs redo (2) Update the numbers}}
\vspace{-1pc}
\label{tab:results-by-length}
\end{table*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}

\iffalse
\begin{table*}[t]
\centering
\small
\addtolength{\tabcolsep}{-0.8mm}
\begin{tabular}{@{}llcccccccccccc@{}}
\toprule
\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Text\\ Length\\ (\#word)\end{tabular}}} & \multirow{3}{*}{\textbf{Model}} & \multicolumn{6}{c}{\textbf{ACC} $\uparrow$} & \multicolumn{6}{c}{\textbf{MSE} $\downarrow$} \\ \cmidrule(lr){3-8} \cmidrule(lr){9-14}
 &  & \multicolumn{2}{c}{\textbf{structured}} & \multicolumn{2}{c}{\textbf{plain}} & \multicolumn{2}{c}{\textbf{shuffled}} & \multicolumn{2}{c}{\textbf{structured}} & \multicolumn{2}{c}{\textbf{plain}} & \multicolumn{2}{c}{\textbf{shuffled}} \\ \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12} \cmidrule(lr){13-14}
 &  & \textbf{tw} & \textbf{cn} & \textbf{tw} & \textbf{cn} & \textbf{tw} & \textbf{cn} & \textbf{tw} & \textbf{cn} & \textbf{tw} & \textbf{cn} & \textbf{tw} & \textbf{cn} \\ \midrule
\multirow{6}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Short\\ (1-49)\end{tabular}}} 
 & \textbf{GPT-4o} & \cellcolor{lightred}0.265 & 0.274 & 0.192 & \cellcolor{lightblue}0.208 & 0.186 & 0.202 & 3.563 & 3.769 & \cellcolor{lightgreen}4.092 & 3.856 & 4.347 & 3.561 \\
 & \textbf{Llama3 8b} & 0.234 & 0.216 & \textbf{0.176} & 0.184 & \textbf{0.162} &0.169. & \textbf{3.402} & 3.931 & \textbf{3.059} & 2.851 & \textbf{3.220} & 3.071 \\
 & \textbf{Llama3 70b} & 0.392 & 0.399 & 0.297 &0.310 & 0.288 & 0.310 & 1.785 & 1.661 & 3.465 & 3.005 & 3.427 & 2.941 \\
 & \textbf{Llama3 405b} & \textbf{0.386} & 0.412 & \textbf{0.283} & 0.315 & \textbf{0.290} & 0.322 & \textbf{2.605} & 2.430 & \textbf{4.365} & 3.598 & \textbf{4.355} & 3.612 \\
 & \textbf{Gemma2 9b} &0.150 & \textbf{0.138} &\textbf{0.182} & 0.193 & \textbf{0.171} & 0.184 & 2.987 & \textbf{3.168} & \textbf{4.089} & 3.367 & \textbf{4.462} & 3.646 \\
 & \textbf{Gemma2 27b} & 0.109 & 0.109 & 0.122 & 0.124 & 0.122 & 0.127 & \textbf{5.399} & 5.120 & \textbf{6.150} & 5.292 & \textbf{5.880} & 5.183 \\ \midrule
\multirow{6}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Long\\ (50+)\end{tabular}}} 
 & \textbf{GPT-4o} & 0.356 & \cellcolor{lightyellow}0.384 & 0.281 & 0.332 & \cellcolor{lightgreen}0.267 & 0.314 & 1.846 & 1.577 & 1.834 & \cellcolor{lightred}1.570 & 2.070 & 1.743 \\
 & \textbf{Llama3 8b} & 0.224 & 0.228 & 0.189 & 0.214 & 0.179 & 0.200 & 1.895 & 1.901 & 2.024 & 1.835 & 2.111 & 1.933 \\
 & \textbf{Llama3 70b} & \textbf{0.409} & 0.435 & \textbf{0.373} & 0.391 & \textbf{0.360} & 0.388 & \textbf{1.424} & 1.284 & \textbf{1.667} & 1.557 & \textbf{1.771} & 1.608 \\
 & \textbf{Llama3 405b} & \textbf{0.380} & 0.410 & \textbf{0.371} & 0.396 & \textbf{0.357} & 0.384 & \textbf{1.866} & 1.627 & \textbf{1.906} & 1.719 & \textbf{2.052} & 1.844 \\
 & \textbf{Gemma2 9b} & 0.142 & 0.151 & \textbf{0.192} & 0.209 & \textbf{0.174} & 0.188 & \textbf{2.515} & 2.350 & \textbf{2.144} & 1.979 & \textbf{2.399} & 2.193 \\
 & \textbf{Gemma2 27b} & 0.096 & 0.092 & 0.077 & 0.075 & 0.079 & 0.083 & \textbf{5.135} & 4.919 & \textbf{5.913} & 5.578 & \textbf{5.606} & 5.160 \\ \midrule
\multirow{6}{*}{\textbf{Overall}} 
 & \textbf{GPT-4o} & 0.296 & 0.312 & \cellcolor{lightblue}0.222 & 0.250 & 0.213 & \cellcolor{lightyellow}0.240 & 2.978 & 3.022 & 3.323 & 2.767 & \cellcolor{lightred}3.571 & 2.942 \\
 & \textbf{Llama3 8b} &0.230 & 0.221 & 0.181 & 0.195 & 0.168 & 0.181 & 2.838 & 3.170 &2.672 & 2.470 & 2.806 & 2.644 \\
 & \textbf{Llama3 70b} & \textbf{0.398} & 0.412 & \textbf{0.324} & 0.339 & \textbf{0.313} & 0.337 & \textbf{1.658} & 1.529 & \textbf{2.835} & 2.496 & \textbf{2.847} & 2.473 \\
 & \textbf{Llama3 405b} & \textbf{0.384} & 0.411 & \textbf{0.314} & 0.344 & \textbf{0.313} & 0.344 & \textbf{2.347} & 2.148 & \textbf{3.505} & 2.939 & \textbf{3.550} & 2.992 \\
 & \textbf{Gemma2 9b} & 0.147 & 0.143 & \textbf{0.185} & 0.199 & \textbf{0.172} & 0.186 & 2.823 & 2.882 & \textbf{3.410} & 2.881 & \textbf{3.742} & 3.137 \\
 & \textbf{Gemma2 27b} & 0.105 & 0.103 & 0.106 & 0.107 & 0.107 & 0.111 & \textbf{5.307} & 5.049 & \textbf{6.067} & 5.392 & \textbf{5.785} & 5.175 \\ \bottomrule

\end{tabular}
\addtolength{\tabcolsep}{+0.8mm}
\caption{Results by length for GPT-4o, Llama3 (8b, 70b, 405b), and Gemma2 (9b, 27b) models. Bold numbers indicate a significant difference between the groups. \cy{I would prefer to us * to represent the significance. The number of stars is also important to report.}}
\label{tab:results-by-length}
\end{table*}
\fi

% 
\iffalse
\begin{table*}[t]
\centering
\small
\addtolength{\tabcolsep}{-0.5mm}
\begin{tabular}{@{}llcccccccccccc@{}}
\toprule
\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Text\\ Length\\ (\#word)\end{tabular}}} & \multirow{3}{*}{\textbf{Model}} & \multicolumn{6}{c}{\textbf{ACC}} & \multicolumn{6}{c}{\textbf{MSE}} \\ \cmidrule(lr){3-8} \cmidrule(lr){9-14}
 &  & \multicolumn{2}{c}{\textbf{structured}} & \multicolumn{2}{c}{\textbf{plain}} & \multicolumn{2}{c}{\textbf{shuffled}} & \multicolumn{2}{c}{\textbf{structured}} & \multicolumn{2}{c}{\textbf{plain}} & \multicolumn{2}{c}{\textbf{shuffled}} \\ \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12} \cmidrule(lr){13-14}
 &  & \textbf{tw} & \textbf{cn} & \textbf{tw} & \textbf{cn} & \textbf{tw} & \textbf{cn} & \textbf{tw} & \textbf{cn} & \textbf{tw} & \textbf{cn} & \textbf{tw} & \textbf{cn} \\ \midrule
\multirow{6}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Short\\ (1-50)\end{tabular}}} 
 & \textbf{GPT-4o} & 0.265 & 0.274 & 0.192 & 0.208 & 0.186 & 0.202 & 3.563 & 3.769 & 4.092 & 3.856 & 4.347 & 3.561 \\
 & \textbf{Llama3 8b} & . & . & . & . & . & . & . & . & . & . & . & . \\
 & \textbf{Llama3 70b} & . & . & . & . & . & . & . & . & . & . & . & . \\
 & \textbf{Llama3 405b} & . & . & . & . & . & . & . & . & . & . & . & . \\
 & \textbf{Gemma2 9b} & . & . & . & . & . & . & . & . & . & . & . & . \\
 & \textbf{Gemma2 27b} & . & . & . & . & . & . & . & . & . & . & . & . \\ \midrule
\multirow{6}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Long\\ (51+)\end{tabular}}} 
 & \textbf{GPT-4o} & 0.356 & 0.384 & 0.281 & 0.332 & 0.267 & 0.314 & 1.846 & 1.577 & 1.834 & 1.570 & 2.070 & 1.743 \\
 & \textbf{Llama3 8b} & . & . & . & . & . & . & . & . & . & . & . & . \\
 & \textbf{Llama3 70b} & . & . & . & . & . & . & . & . & . & . & . & . \\
 & \textbf{Llama3 405b} & . & . & . & . & . & . & . & . & . & . & . & . \\
 & \textbf{Gemma2 9b} & . & . & . & . & . & . & . & . & . & . & . & . \\
 & \textbf{Gemma2 27b} & . & . & . & . & . & . & . & . & . & . & . & . \\ \midrule
\multirow{6}{*}{\textbf{Overall}} 
 & \textbf{GPT-4o} & 0.296 & 0.312 & 0.222 & 0.250 & 0.213 & 0.240 & 2.978 & 3.022 & 3.323 & 2.767 & 3.571 & 2.942 \\
 & \textbf{Llama3 8b} & . & . & . & . & . & . & . & . & . & . & . & . \\
 & \textbf{Llama3 70b} & . & . & . & . & . & . & . & . & . & . & . & . \\
 & \textbf{Llama3 405b} & . & . & . & . & . & . & . & . & . & . & . & . \\
 & \textbf{Gemma2 9b} & . & . & . & . & . & . & . & . & . & . & . & . \\
 & \textbf{Gemma2 27b} & . & . & . & . & . & . & . & . & . & . & . & . \\ \bottomrule
\end{tabular}
\addtolength{\tabcolsep}{+0.5mm}
\caption{Results by length for GPT-4o, Llama3 (8b, 70b, 405b), and Gemma2 (9b, 27b) models.}
\label{tab:results-by-length}
\end{table*}
\fi

\begin{comment}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[t]
\centering
\footnotesize
\begin{tabular}{@{}llcccccccccccc@{}}
\toprule
\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Text\\ Length\\ (\#word)\end{tabular}}} & \multirow{3}{*}{\textbf{Model}} & \multicolumn{6}{c}{\textbf{ACC}} & \multicolumn{6}{c}{\textbf{MSE}} \\ \cmidrule(l){3-14} 
 &  & \multicolumn{2}{c}{\textbf{structured}} & \multicolumn{2}{c}{\textbf{plain}} & \multicolumn{2}{c}{\textbf{shuffled}} & \multicolumn{2}{c}{\textbf{structured}} & \multicolumn{2}{c}{\textbf{plain}} & \multicolumn{2}{c}{\textbf{shuffled}} \\ \cmidrule(l){3-14} 
 &  & \textbf{tw} & \textbf{cn} & \textbf{tw} & \textbf{cn} & \textbf{tw} & \textbf{cn} & \textbf{tw} & \textbf{cn} & \textbf{tw} & \textbf{cn} & \textbf{tw} & \textbf{cn} \\ \midrule
\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Short\\ (1-49)\end{tabular}}} & \textbf{GPT4o} & .265 & .274 & .192 & .208 & .186 & .202 & 3.563 & 3.769 & 4.092 & 3.856 & 4.347 & 3.561 \\
 & \textbf{Llama3} & .MMM & .NNN & .OOO & .PPP & .QQQ & .RRR & .MMM & .NNN & .OOO & .PPP & .QQQ & .RRR \\
 & \textbf{Gemma2} & .SSS & .TTT & .UUU & .VVV & .XXX & .YYY & .SSS & .TTT & .UUU & .VVV & .XXX & .YYY \\ \midrule
\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Long\\ (50+)\end{tabular}}} & \textbf{GPT} & .356 & .384 & .281 & .332 & .267 & .314 & 1.846 & 1.577 & 1.834 & 1.570 & 2.070 & 1.743 \\
 & \textbf{Llama} & .MMM & .NNN & .OOO & .PPP & .QQQ & .RRR & .MMM & .NNN & .OOO & .PPP & .QQQ & .RRR \\
 & \textbf{Gemma2} & .SSS & .TTT & .UUU & .VVV & .XXX & .YYY & .SSS & .TTT & .UUU & .VVV & .XXX & .YYY \\ \midrule
\multirow{3}{*}{\textbf{Overall}} & \textbf{GPT} & .296 & .312 & .222 & .250 & .213 & .240 & 2.978 & 3.022 & 3.323 & 2.767 & 3.571 & 2.942 \\
 & \textbf{Llama} & .MMM & .NNN & .OOO & .PPP & .QQQ & .RRR & .MMM & .NNN & .OOO & .PPP & .QQQ & .RRR \\
 & \textbf{Gemma2} & .SSS & .TTT & .UUU & .VVV & .XXX & .YYY & .SSS & .TTT & .UUU & .VVV & .XXX & .YYY \\ \bottomrule
\end{tabular}
\caption{Results by length.\kenneth{TODO: List (1) GPT-4o, (2) Llama3 8b, (3) Llama3 70b, (4) Gemma2 9b, (5) Llama3 405b, (6) Gemma2 27b}}
\label{tab:results-by-length}
\end{table*}
\end{comment}

\begin{comment}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[t]
\centering
%\small

\iffalse
\begin{tabular}{@{}llcccc@{}}
\toprule
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Text\\ Length\end{tabular}}} & \multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c}{\textbf{ACC}} & \multicolumn{2}{c}{\textbf{MSE}} \\ \cmidrule(l){3-6} 
 &  & \textbf{tw} & \textbf{ch} & \textbf{tw} & \textbf{ch} \\ \midrule
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Short (0-50 words)\\ n=A,AA\end{tabular}}} & \textbf{GPT-4o} & .264, .191, .185 & .273, .206, .200 & E.EE & F.FF \\
 & \textbf{LLaMA 3.1} & .AAA & .BBB & E.EE & F.FF \\ \midrule
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Medium (50-270 words)\\ n=B,BB\end{tabular}}} & \textbf{GPT-4o} & .355, .280, .266 & .383, .331, .313 & E.EE & F.FF \\
 & \textbf{LLaMA 3.1} & .AAA & .BBB & E.EE & F.FF \\ \midrule
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Long (270+ words)\\ n=C,CC\end{tabular}}} & \textbf{GPT-4o} & .002, .001, .001 & .001, .001, .001 & E.EE & F.FF \\
 & \textbf{LLaMA 3.1} & .AAA & .BBB & E.EE & F.FF \\ \midrule
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Overall\\ n=D,DD\end{tabular}}} & \textbf{GPT-4o} & .296, .222, .213 & .312, .250, .240 & E.EE & F.FF \\
 & \textbf{LLaMA 3.1} & .AAA & .BBB & E.EE & F.FF \\ \bottomrule
\end{tabular}
\fi

\end{table*}
\end{comment}



\begin{comment}



% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[t]
\centering
\small
\begin{tabular}{@{}llcccccccc@{}}
\toprule
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Text\\ Length\end{tabular}}} & \multirow{2}{*}{\textbf{LLMs}} & \multicolumn{4}{c}{\textbf{ACC}} & \multicolumn{4}{c}{\textbf{MSE}} \\ \cmidrule(l){3-10} 
 &  & \textbf{tw} & \textbf{ch} & \textbf{tw-\textgreater{}ch} & \textbf{ch-\textgreater{}tw} & \textbf{tw} & \textbf{ch} & \textbf{tw-\textgreater{}ch} & \textbf{ch-\textgreater{}tw} \\ \midrule
\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Short\\ (0-50 words)\\ n=A,AA\end{tabular}}} & \textbf{GPT-4o} & .AAA & .BBB & .CCC & .DDD & E.EE & F.FF & G.GG & H.HH \\
 & \textbf{OpenAI o1} & .AAA & .BBB & .CCC & .DDD & E.EE & F.FF & G.GG & H.HH \\
 & \textbf{LLaMA 3.1} & .AAA & .BBB & .CCC & .DDD & E.EE & F.FF & G.GG & H.HH \\ \midrule
\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Medium\\ (50-300 words)\\ n=B,BB\end{tabular}}} & \textbf{GPT-4o} & .AAA & .BBB & .CCC & .DDD & E.EE & F.FF & G.GG & H.HH \\
 & \textbf{OpenAI o1} & .AAA & .BBB & .CCC & .DDD & E.EE & F.FF & G.GG & H.HH \\
 & \textbf{LLaMA 3.1} & .AAA & .BBB & .CCC & .DDD & E.EE & F.FF & G.GG & H.HH \\ \midrule
\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Long\\ (300+ words)\\ n=C,CC\end{tabular}}} & \textbf{GPT-4o} & .AAA & .BBB & .CCC & .DDD & E.EE & F.FF & G.GG & H.HH \\
 & \textbf{OpenAI o1} & .AAA & .BBB & .CCC & .DDD & E.EE & F.FF & G.GG & H.HH \\
 & \textbf{LLaMA 3.1} & .AAA & .BBB & .CCC & .DDD & E.EE & F.FF & G.GG & H.HH \\ \midrule
\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Overall\\ n=D,DD\end{tabular}}} & \textbf{GPT-4o} & .AAA & .BBB & .CCC & .DDD & E.EE & F.FF & G.GG & H.HH \\
 & \textbf{OpenAI o1} & .AAA & .BBB & .CCC & .DDD & E.EE & F.FF & G.GG & H.HH \\
 & \textbf{LLaMA 3.1} & .AAA & .BBB & .CCC & .DDD & E.EE & F.FF & G.GG & H.HH \\ \bottomrule
\end{tabular}
\caption{Results by length.}
\label{tab:results-by-length}
\end{table*}
    
\end{comment}
